Data Science and Machine Learning in Education

The growing role of data science (DS) and machine learning (ML) in high-energy physics (HEP) is well established and pertinent given the complex detectors, large data, sets and sophisticated analyses at the heart of HEP research. Moreover, exploiting symmetries inherent in physics data have inspired physics-informed ML as a vibrant sub-field of computer science research. HEP researchers benefit greatly from materials widely available materials for use in education, training and workforce development. They are also contributing to these materials and providing software to DS/ML-related fields. Increasingly, physics departments are offering courses at the intersection of DS, ML and physics, often using curricula developed by HEP researchers and involving open software and data used in HEP. In this white paper, we explore synergies between HEP research and DS/ML education, discuss opportunities and challenges at this intersection, and propose community activities that will be mutually beneficial.

==> header.tex <==
% Packages
%***************
\RequirePackage{lineno}\newdimen\linenumbersep\linenumbersep=2pt\renewcommand{\linenumberfont}{\tiny\color{lightgray}}
\usepackage{amsmath, amsfonts, amssymb, booktabs, color, eurosym, fancyhdr, graphicx, lastpage, layout, multicol, pbox, pdfpages, url, verbatim, xspace, tabularx, wrapfig}
\usepackage[table,xcdraw,usenames,dvipsnames]{xcolor}
\usepackage[font={small},bf]{caption}
\usepackage[colorlinks=true,citecolor=black,filecolor=black,linkcolor=black,urlcolor=black,pdftex]{hyperref}
\usepackage{lipsum}  
\usepackage{units}
\usepackage{paralist}
\usepackage{multirow}
\usepackage{xspace}
\usepackage[normalem]{ulem}
\usepackage{mathptmx}
\usepackage[compact]{titlesec}
\usepackage{paralist}
\usepackage{todonotes}
\usepackage{enumitem}
\usepackage{parskip}
%\usepackage[redeflists]{IEEEtrantools}
%\usepackage[
%backend=biber,
%style=numeric,
%maxnames=50,
%citestyle=ieee
%]{biblatex}

\usepackage[style=numeric-comp,sorting=none,backend=biber,maxbibnames=90,bibencoding=utf8]{biblatex}

\usepackage[capitalize]{cleveref}% https://ctan.org/pkg/cleveref % Must be loaded after hyperref
\creflabelformat{equation}{#2\textup{#1}#3}% Equation references don't have parentheses  

%***************
% Formatting
%***************
% 8.5 x 11 inch is standard US letter size
% PAPPG requires inch on every side
% https://www.nsf.gov/pubs/policydocs/pappg17_1/pappg_2.jsp#IIB2
% so 8.5-2=6.5 and 11-2=9
\setlength{\textheight}{9.0in}
\setlength{\textwidth}{6.5in}
\setlength{\topmargin}{0mm}
\setlength{\oddsidemargin}{0mm}
\setlength{\evensidemargin}{0mm}
\setlength{\headheight}{0pt}
\setlength{\headsep}{0pt}
%\setlength{\textfloatsep}{2pt}
\setlength{\textfloatsep}{0pt}

\titlespacing{\section}{0pt}{2ex}{1ex}
\titlespacing{\subsection}{0pt}{1ex}{0ex}
\titlespacing{\subsubsection}{0pt}{0.5ex}{0ex}
\titleformat{\subsubsection}[runin]{\bfseries}{\thesubsubsection~}{0.5em}{}[:~ ]

\newenvironment{itemize*}{
   \begin{list}
   {\labelitemiv}{ % \labelitemi is standard
   \setlength{\topsep}{0mm}        % amount of extra vertical space at top of list
   \setlength{\partopsep}{0mm}     % extra length at top if environment is preceded by a blank line (should be a rubber length)
   \setlength{\itemsep}{1mm}       % amount of extra vertical space between items
   \setlength{\parsep}{0mm}        % amount of vertical space between paragraphs within an item
   \setlength{\leftmargin}{3mm}    % horizontal distance between the left margins of the environment and the list; must be nonnegative
   \setlength{\rightmargin}{0mm}   % horizontal distance betwen the right margins of the enviroment and the list; must be nonnegative
   \setlength{\listparindent}{0mm} % amount of extra space for paragraph indent after the first in an item; can be negative
   \setlength{\parskip}{0mm}
}}{\end{list}}
%***************

\newcounter{junk}
\newenvironment{denseitemize}{ \begin{list}{$\bullet$}
                               {\usecounter{junk}
                                \setlength\itemsep{-1mm}
                              \setlength\leftmargin{6mm}
                                \setlength\topsep{0mm}}}
                               {\end{list}}
\newenvironment{itemizenoindent}{ \begin{list}{$\bullet$}
                               {\usecounter{junk}
                              \setlength\itemsep{-0.5mm}
                           \setlength\leftmargin{3mm}
                                \setlength\topsep{0mm}}}
                               {\end{list}}

% setting a new caption that would work in two columns of figures.
\newcommand{\mycaption}[1]{\refstepcounter{figure}{\bf Figure \arabic{figure}}: #1}

% Proposal title and short footer
%***************
\newcommand{\actualtitle}{\large{\textbf{\emph{Elements: Development of Modular and Sustainable Cyberinfrastructure for Matrix Element Analyses}}}}
\pagestyle{fancy}\fancyhf{}

\sloppy
%***************

% Commands, macros, notation, etc.
%***************
\renewcommand{\headrulewidth}{0pt}

\newcommand{\etal}{{\it et al.}}
\newcommand\note[2]{{\color{blue}[#1: #2]}}


